Optimized Wireless Control and Telemetry Network for Mobile Soccer Robots

In a diverse set of robotics applications, including RoboCup categories, mobile robots require control commands to interact with surrounding environment correctly. These control commands should come wirelessly to not interfere in robots' movement; also, the communication has a set of requirements, including low latency and consistent delivery. This paper presents a complete communication architecture consisting of computer communication with a base station, which transmits the data to robots and returns robots telemetry to the computer. With the proposed communication, it is possible to send messages in less than 4.5ms for six robots with telemetry enables in all of them.

==> equations/avg.tex <==
\begin{equation}
\label{eq:avg}
time_{interval} = \frac{\sum_{i = 1}^{500}{(messageTime_i - messageTime_{i-1})}}{500}
\end{equation}


==> equations/std.tex <==
\begin{equation}
\label{eq:std}
s_{interval} = \sqrt{\frac{1}{499} \sum_{i = 1}^{500}(messageTime_i - messageTime_{i-1})}
\end{equation}

==> figures/architecture.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.8\linewidth]{figures/architecture.png}
	\caption{\textmd{Base station architecture of the proposed wireless network with Serial and Ethernet options between the Computer and Base Station}.}
	\label{fig:architecture}
\end{figure}


==> figures/architectureOverview.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figures/architectureOverview.png}
	\caption{\textmd{Project network overview with a computer that sends commands to a base station
which transmits the message wirelessly to multiple robots and they are sending telemetry back to the commander.}.}
	\label{fig:OverviewComm}
\end{figure}

==> figures/basestation.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.6\linewidth]{figures/basestation.jpg}
	\caption{\textmd{Proposed Base Station hardware}.}
	\label{fig:basestation}
\end{figure}


==> figures/results/delivery.tex <==
\begin{figure}
    \centering
    \captionsetup[subfloat]{justification=centering}
    \subfloat[Serial station with 1900us of interval]{\includegraphics[width=.45\linewidth, scale=1]{figures/results/delivery-ser.png}}
    \label{fig:delivery-ser}
    \subfloat[Ethernet station with 500us of interval]{\includegraphics[width=.45\linewidth, scale=1]{figures/results/delivery-eth.png}}
    \label{fig:delivery-eth}
    
	\caption{\textmd{Delivery time of base station approaches with the minimum sending interval}.}
	\label{fig:delivery}
\end{figure}

==> figures/results/eth-interval.tex <==
\begin{figure}
	\centering
	\includegraphics[width=.5\linewidth]{figures/results/eth-interval.png}
	\caption{\textmd{Reception delay for 30 tests at each different sending interval, using a Ethernet base station transmitting computer messages at the configured sending intervals}.}
	\label{fig:eth-interval}
\end{figure}


==> figures/results/multiple-compare.tex <==
\begin{figure}[H]
    \centering
    \captionsetup[subfloat]{justification=centering}
    \subfloat[Delivery time of Ethernet base station at two robots network\label{fig:mult-comp-2r}]{\includegraphics[width=.45\linewidth, scale=1]{figures/results/multiple-comp-2r.png}}
    \subfloat[Delivery time of 6 robots network with Ethernet base station at two nodes\label{fig:mult-comp-6r}]{\includegraphics[width=.45\linewidth, scale=1]{figures/results/multiple-comp-6r.png}}
	\caption{\textmd{Comparing delivery time with two and six nodes network at two different robots}.}
	\label{fig:multp-compare}
\end{figure}


==> figures/results/serial-interval.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{figures/results/serial-interval.png}
	\caption{\textmd{Reception delay for 30 tests at each different sending interval, using a Serial base station transmitting computer messages at the configured sending intervals}.}
	\label{fig:serial-interval}
\end{figure}


==> figures/results/telemetry-interval.tex <==
\begin{figure}[H]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/results/telemetry-interval.png}
	\caption{\textmd{Delivery time of Ethernet base station packets with different telemetry sampling time}.}
	\label{fig:telemetry}
\end{figure}


==> figures/results/telemetry-mult.tex <==
\begin{figure}[H]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/results/telemetry-mult.png}
	\caption{\textmd{Delivery time of Ethernet base station packets with different telemetry sampling time at 6 robots control network}.}
	\label{fig:telemetry-mult}
\end{figure}


==> figures/ssl-arch.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figures/ssl-arch.png}
	\caption{\textmd{General Structure of the Small Size League Competition Autonomous System \cite{ssl-future}}.}
	\label{fig:ssl-arch}
\end{figure}


==> figures/ssl-robot.tex <==
\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{figures/ssl-robot.jpg}
	\caption{\textmd{RobôCIn's \acrfull{ssl} robot}.}
	\label{fig:ssl-robot}
\end{figure}


==> figures/test-method.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figures/test-method.png}
	\caption{\textmd{Architecture of the method developed for testing the network configurations and interfaces}.}
	\label{fig:test-method}
\end{figure}

